Towards Arabic Multimodal Dataset for Sentiment Analysis

Multimodal Sentiment Analysis (MSA) has recently become a centric research direction for many real-world applications. This proliferation is due to the fact that opinions are central to almost all human activities and are key influencers of our behaviors. In addition, the recent deployment of Deep Learning-based (DL) models has proven their high efficiency for a wide range of Western languages. In contrast, Arabic DL-based multimodal sentiment analysis (MSA) is still in its infantile stage due, mainly, to the lack of standard datasets. In this paper, our investigation is twofold. First, we design a pipeline that helps building our Arabic Multimodal dataset leveraging both state-of-the-art transformers and feature extraction tools within word alignment techniques. Thereafter, we validate our dataset using state-of-the-art transformer-based model dealing with multimodality. Despite the small size of the outcome dataset, experiments show that Arabic multimodality is very promising

==> Tables/IEMOCAP.tex <==
\begin{center}
			\begin{tabular}{|c|c|C{0.6cm}|C{0.6cm}|C{0.6cm}|C{0.6cm}|C{0.6cm}|C{0.6cm}|C{0.6cm}|C{0.6cm}|}
				\cline{3-9}
                \multicolumn{2}{c|}{}&\multicolumn{7}{c|}{Modalities}\\\cline{3-9}
				\multicolumn{2}{c|}{}		 &T	   &  A   &  V      & TA    & TV & AV &  TVA  \\\hline 
				 \multirow{4}{*}{IEMOCAP}  & F1  &  0.646&  0.659 & 0.646  & 0.64  & 0.65  & 0.649  &0.66 \\ 
			    	  &    Accu  &     0.749 &   0.752   &   0.749  & 0.749    &   0.74    &0.74   & 0.76 \\
          & F1  &  0.7654 &  0.7903  &  0.6776 & 0.7871  &  0.7655 &  0.7778  & 0.8087\\ 
			    	  &    Accu  &  0.7750     & 0.7985     &  0.7515    &      0.7960 &   0.7769     &  0.7851 & 0.8163  \\
				  \hline
				   \multirow{2}{*}{UR-FUNNY}  & F1  & 0.671 &  0.569  &  0.563  & 0.681  &   0.666&  0.566  &0.679 \\ 
			    	  &    Accu  & 0.668  &  0.568 &   0.553 &   0.679   &  0.658    &  0.56 & 0.678 \\ 
          
				  \hline
			\end{tabular}
\end{center}

 % FUNNY &    Prams  &  1179393     &     & 1179393   & 1179393    &      &  1179393 & 1220545 \\

==> Tables/M-HS-Performances.tex <==
		\begin{center}
			\begin{tabular}{|c|c|C{0.6cm}|C{0.6cm}|C{0.6cm}|}
				\cline{3-5}
                \multicolumn{2}{c|}{}&\multicolumn{3}{c|}{Modalities}\\\cline{3-5}
				\multicolumn{2}{c|}{} &  T  & I      & TI       \\\hline 
               \multirow{2}{*}{ Hate Memes}  &  Accu     &    59.2  &  55.92  &  68.20  \\  
			  & AUROC    &   65.08   &  52.13   & 74.75    \\\hline		
               \multirow{2}{*}{ MMHS150K    }     &  Accu     &   67.4  & 56.8  &  68.4 \\ 
			  & AUROC    &  72.3  &    58.6    & 73.4   \\\hline	
     
			\end{tabular}
		\end{center}

  %Train loss: 0.0175 Val loss: 0.8440 Val acc: 0.6300 AUC: 0.7369
  
  % rain loss: 0.0099 Val loss: 0.7395 Val acc: 0.3588 AUC: 0.7529
%{"eval_loss": 0.7482683278827204, "eval_macro_f1": 0.728436068171444, "eval_micro_f1": 0.8818493150684931, "learning_rate": 1.32398753894081e-06, "training_loss": 0.48504671663045884, "step": 625}
  

==> Tables/M-MClass-Performances.tex <==
\begin{tabular}{L{1cm}L{2cm}L{1.6cm}L{2.4cm}}
\toprule

 Mertic &	Text  & Image & Image + text   \\\midrule
BLUE  &    37.8  &  36.5   &   39 \\\midrule
METEOR   &    55.3   &  54  &  56.4 \\\midrule
    $\Delta \% \approx $ &   96\%  &     93\%   & 100\% \\\midrule
 
\bottomrule
\end{tabular}



==> Tables/M-SA-Performances.tex <==
		\begin{center}
			\begin{tabular}{|c|c|C{0.8cm}|C{0.8cm}|C{0.8cm}|C{0.8cm}|}
				\cline{3-6}
            
				\multicolumn{2}{c|}{}		 &Text	   &  Audio   &  Video      &  TVA  \\\hline 
				 \multirow{3}{*}{Mult}&  Accu &53.84     &    41.61  &  48.07 &63.46 \\ 
				  &  F1 &    54.46    &   41.45 &   55.10   &   63.80 \\
      &  MAE &     0.85   &  0.98    &    0.83  &0.81\\
   
      \hline
	\multirow{3}{*}{LF-LSTM}&  Accu & 57    &    53.90  & 57.10 &58.73 \\ 
				  &  F1 & 56.60        &  52.90     &   55.60     &  58.90 \\
      &  MAE &  0.83      &  0.83   &     0.88  & 0.81\\
      \hline
			\end{tabular}
		\end{center}


==> Tables/M-Translation.tex <==
\begin{tabular}{L{1cm}L{2cm}L{1.8cm}L{1.5cm}}
\toprule

 Mertic &	Text (MLPW2V) & Image(VGG)	& MMU   \\\midrule
	Micro    &  0.595  & 0.437   &  0.630  \\\midrule
	Macro     & 0.488 & 0.284  &0.541 \\\midrule
             $\Delta \% \approx $        &   90 \% &     AVG 60.4  \%  &  100\%\\\midrule
 
\bottomrule
\end{tabular}

==> Tables/M-food.tex <==
 \begin{tabular}{L{1cm}L{2cm}L{1.8cm}L{1.5cm}}
\toprule

 Mertic &	Text & Image	& Multimodal   \\\midrule
	Accuracy    & 84.41   & 	 71.67 & 92.50 \\\midrule
	
 
\bottomrule
\end{tabular}

==> Tables/M-pairs.tex <==
		\begin{center}
			\begin{tabular}{|c|C{1.6cm} C{1.6cm}|c}
				\cline{2-3}
              
				\multicolumn{1}{c|}{ $\Delta \% $ } &  Text/Audio  & Text/video              \\\cline{1-3} 
               \multirow{2}{*}{ CMU-MOSEI} & 30 \%     &  27\% & A \\
                   &    15\% &   19 \% & UA  \\\cline{1-3}
               \multirow{2}{*}{CMU-MOSI } &  34.8  \%    &  62.11\%   & A   \\
                    &     43\%  &  35.8\%  & UA \\\cline{1-3}
                \multirow{2}{*}{ IEMOCAP} &    -3\%    & 3.1\% & A   \\
                    &  -0.4 \%  & 0 \%  & UA  \\\cline{1-3}
               \multirow{1}{*}{ UR-FUNNY} &   16  \%  &  17\%   \\		
               \multirow{1}{*}{ MMHS150K} &     -  &  18.6  \% \\ 	
               \multirow{1}{*}{ HATEMEMES} &      -&  5.8\%   \\ 	
               \multirow{1}{*}{ FOOD101} &    -  & 17 \%   \\ 	
               \multirow{1}{*}{ MM-IMB} &     - & 50 \%   \\	
                \multirow{1}{*}{Multi30k } &   -   &  3 \%  \\\cline{1-3}	
			\end{tabular}
		\end{center}
 

==> Tables/dataSet-MT.tex <==
\begin{tabular}{L{2cm}L{1.5cm}L{1.5cm}L{4cm}}
\toprule

 Dataset &	Text & Image	& Image & Text   \\\midrule
	BLUE       & 36.75  & 4 & 40 \\\midrule
	METEOR       & 54.95  & 4 &57 \\\midrule

\bottomrule
\end{tabular}


==> Tables/datasets-ER.tex <==
\begin{tabular}{L{2cm}L{1.5cm}L{1.5cm}L{1.5cm}L{4cm}}
\toprule

 Dataset &	Text & Audio	& Video & Available  Pre-processing   \\\midrule
CMU-MOSI\cite{zadeh2018multimodal}	         & & &\\\midrule
IEMOCAP\cite{busso2008iemocap }    & & &\\\midrule

\bottomrule
\end{tabular}


==> Tables/datasets-HateSpeech.tex <==
\begin{tabular}{L{2cm}L{1.5cm}L{1.5cm}L{1.5cm}L{4cm}}
\toprule

 Dataset &	Text & Audio	& Video & Available  Pre-processing   \\\midrule
Hate speech memes \cite{kiela2020hateful }       & & &\\\midrule


\bottomrule
\end{tabular}


==> Tables/datasets-QA.tex <==
\begin{tabular}{L{2cm}L{1.5cm}L{1.5cm}L{1.5cm}L{4cm}}
\toprule

 Dataset &	Text & Audio	& Video & Available  Pre-processing   \\\midrule
CMU-MOSI\cite{zadeh2018multimodal}	       & & &\\\midrule


\bottomrule
\end{tabular}

==> Tables/datasets-SA.tex <==
\begin{tabular}{L{2cm}L{2cm}L{1.5cm}L{1.5cm}L{1.5cm}L{4cm}L{2cm}}
\toprule

 Tasks & Dataset &	Text & Audio	& Video & Available  Pre-processing &  Details\\\midrule
\multirow{2}{*}{}CMU-MOSI\cite{zadeh2016mosi}    & & &\\\midrule
CMU-MOSEI\cite{zadeh2018multimodal }     & 63727 sentence & &90.23h &  16514 videos\\\midrule

\bottomrule
\end{tabular}


==> Tables/datasets.tex <==
\begin{tabular}{L{2cm}L{2cm}L{1.5cm}L{1.5cm}L{1.5cm}L{4cm}L{2cm}}
\toprule

 Tasks & Dataset &	Text & Audio	& Video & Available  Pre-processing &  Details\\\midrule
\multirow{2}{*}{M-SA}
&CMU-MOSI\cite{zadeh2016mosi}    & & &\\\cline{2-7}
&CMU-MOSEI\cite{zadeh2018multimodal }     & 63727 sentence & &90.23h &  16514 videos\\\midrule
\multirow{2}{*}{ER} &    & & &\\\cline{2-7}
  
 
    &  & & &   \\

\multirow{2}{*}{M-HS} &  Hate Memes   & & &\\\cline{2-7}
  
 
 MMHS150K   & 63727 sentence & &90.23h &  16514 videos\\\midrule

\multirow{2}{*}{M-Movie Class.} &    & & &\\\cline{2-7}
  
 
    &  & & &  \\\midrule

\multirow{2}{*}{M-Translation} &     & & &\\\cline{2-7}
  
 
    &  & & &   \\\midrule
\multirow{2}{*}{Food Class.} &    & & &\\\cline{2-7}
  
 
    &  & & &   \\
\bottomrule
\end{tabular}


==> Tables/details.tex <==
\begin{tabular}{|L{3cm}|L{3cm}|}
\toprule

 Videos Number  &	10  \\\midrule
	  Total segments     & 25 \\\midrule
	   Total of negative segments  &  \\\midrule
	   Total of positive segments     &  \\\midrule
     Total number of words     & 2485  \\\midrule
\bottomrule
\end{tabular}

==> Tables/ur-funny.tex <==
\begin{tabular}{L{1cm}L{2cm}L{1.6cm}L{2.4cm}}
\toprule

 Mertic &	Text  & Image & Image + text   \\\midrule
	BLUE  &     &    &   39 \\\midrule
	METEOR   &      &    &  56.4 \\\midrule
        $\Delta $\% &     &        & 100\% \\\midrule
 
\bottomrule
\end{tabular}

==> old-ref.tex <==

%Our research will be guided by the goals of improving the robustness and efficiency of multimodal sentiment analysis in Arabic, and exploring the benefits of using multimodal information for sentiment prediction.
%To overcome this challenge, some researchers have attempted to create their own multimodal datasets in Arabic, either by collecting data from social media platforms or by crowd-sourcing annotations. However, these datasets are often small and limited in scope, which can make it challenging to develop and evaluate models with high generalization performance.Given the importance of having access to large and diverse multimodal datasets for advancing the field of Arabic MML, it is crucial for researchers in this area to work towards the creation of publicly available annotated multimodal datasets in Arabic. This can be done through collaboration with institutions, organizations, and communities, as well as through efforts to overcome the technical, ethical, and legal challenges associated with data collection and annotation.%

\bibitem{b1} Al-Shedivat M, Wilson AG, Saatchi Y, Hu Z, Xing EP (2017)
Learning scalable deep Kernels with recurrent structure.
\bibitem{b2} Hofmann T, Schölkopf B, Smola AJ (2008) Kernel methods in
machine learning. Ann Stat 
\bibitem{b3} Nair K.Nikhitha  A.Afzal  S.Asharaf Deep Kernel machines: a survey.  8 June 2019.
\bibitem{b4} Aronszajn N (1950) Theory of reproducing Kernels. Trans Am
Math Soc 
\bibitem{b5} Poria S, Cambria E, Gelbukh A (2015) Deep convolutional neural network textual features and multiple Kernel learning for
utterance-level multimodal sentiment analysis. In: Proceedings
of the 2015 conference on empirical methods in natural language
processing, 

\bibitem{b6} Afzal A, Asharaf S (2018) Deep multiple multilayer Kernel
learning in core vector machines. Expert Syst Appl 96:149–156.
\bibitem{b7} Afzal A, Asharaf S (2017) Deep Kernel learning in core vector
machines. Pattern Anal Appl 21:721

\bibitem{b8} Chen D, Jacob L, Mairal J (2018) Biological sequence modeling with convolutional Kernel networks. bioRxiv p 217257

\bibitem{b9} Shawe-Taylor J, Cristianini N (2004) Kernel methods for pattern
analysis. Cambridge University Press, Cambridge

\bibitem{b10} Charu C. Aggarwal. Neural Networks and Deep Learning. Springer, Cham, 2018

\bibitem{b11} Sutskever I, Hinton G (2010) Temporal-Kernel recurrent neural
networks. Neural Netw 
\bibitem{b12} Slimane Bellaouar. Noyaux de mots et d'arbres : efficacite et unification. PhD thesis,
Universite Amar Telidji-Laghouat, Algerie, 2018. P20

\bibitem{b13} Matthew A. Wright and Joseph E. Gonzalez
Transformers are Deep Infinite-Dimensional Non-Mercer Binary
Kernel Machines
University of California
Berkeley, CA 94705

\bibitem{b14}Marc Peter,Deisenroth, A. Aldo Faisal, Cheng Soon Ong;
MATHEMATICS FOR MACHINE LEARNING by Cambridge University Press 2020

\bibitem{b15}
THOMAS M. COVER, 
Geometrical and Statistical Properties of Systems of
Linear Inequalities with Applications in Pattern
Recognition
\end{thebibliography}

==> transformerTikz.tex <==


\begin{tikzpicture}[scale=0.85]
\definecolor{emb_color}{RGB}{252,224,225}
\definecolor{multi_head_attention_color}{RGB}{252,226,187}
\definecolor{add_norm_color}{RGB}{242,243,193}
\definecolor{ff_color}{RGB}{194,232,247}
\definecolor{softmax_color}{RGB}{203,231,207}
\definecolor{linear_color}{RGB}{220,223,240}
\definecolor{gray_bbox_color}{RGB}{243,243,244}
\draw[fill=gray_bbox_color, line width=0.046875cm, rounded corners=0.300000cm] (-0.975000, 6.455000) -- (2.725000, 6.455000) -- (2.725000, 1.305000) -- (-0.975000, 1.305000) -- cycle;

\draw[line width=0.046875cm, fill=emb_color, rounded corners=0.100000cm] (0.000000, 0.000000) -- (2.500000, 0.000000) -- (2.500000, -0.900000) -- (0.000000, -0.900000) -- cycle;
\node[text width=2.500000cm, align=center] at (1.250000,-0.450000) {Input \vspace{-0.05cm} \linebreak Embedding};m
 
 \draw[line width=0.046875cm, fill=add_norm_color, rounded corners=0.100000cm] (0.000000, 3.730000) -- (2.500000, 3.730000) -- (2.500000,3.180000) -- (0.000000,3.180000) -- cycle;
\node[text width=2.500000cm, align=center] at (1.250000,3.430000) {Add \& Norm};

\draw[line width=0.046875cm, fill=multi_head_attention_color, rounded corners=0.100000cm] (0.000000, 3.030000) -- (2.500000, 3.030000) -- (2.500000, 2.130000) -- (0.000000, 2.130000) -- cycle;
\node[text width=2.500000cm, align=center] at (1.250000,2.580000) {Multi-Head \vspace{-0.05cm} \linebreak Attention};
\draw[line width=0.046875cm] (1.250000, 3.030000) -- (1.250000, 3.180000);
 
 

\draw[line width=0.046875cm] (1.250000, 5.900000) -- (1.250000, 5.730000);

%%%%

\draw[line width=0.046875cm, fill=add_norm_color, rounded corners=0.100000cm] (0.000000, 6.230000) -- (2.500000, 6.230000) -- (2.500000, 5.730000) -- (0.000000, 5.730000) -- cycle;
\node[text width=2.500000cm, align=center] at (1.250000,5.980000) {Add \& Norm};

\draw[line width=0.046875cm, fill=ff_color, rounded corners=0.100000cm] (0.000000, 5.580000) -- (2.500000, 5.580000) -- (2.500000, 4.680000) -- (0.000000, 4.680000) -- cycle;
\node[text width=2.500000cm, align=center] at (1.250000,5.130000) {Feed \vspace{-0.05cm} \linebreak Forward};
 
\draw[line width=0.046875cm, fill=linear_color, rounded corners=0.100000cm] (0.000000, 10.280000) -- (2.500000, 10.280000) -- (2.500000, 9.780000) -- (0.000000, 9.780000) -- cycle;
\node[text width=2.500000cm, align=center] at (1.250000,10.030000) {Linear};
 
\draw[line width=0.046875cm, fill=softmax_color, rounded corners=0.100000cm] (0.000000, 11.380000) -- (2.500000, 11.380000) -- (2.500000, 10.880000) -- (0.000000, 10.880000) -- cycle;
\node[text width=2.500000cm, align=center] at (1.250000,11.130000) {Softmax};
\draw[line width=0.046875cm] (1.250000, 0.600000) circle (0.200000);
\draw[line width=0.046875cm] (1.410000, 0.600000) -- (1.090000, 0.600000);
\draw[line width=0.046875cm] (1.250000, 0.760000) -- (1.250000, 0.440000);
 
\draw[line width=0.046875cm] (0.350000, 0.600000) circle (0.400000);
\draw[line width=0.046875cm] (-0.030000, 0.600000) -- (-0.014490, 0.629156) -- (0.001020, 0.657833) -- (0.016531, 0.685561) -- (0.032041, 0.711884) -- (0.047551, 0.736369) -- (0.063061, 0.758616) -- (0.078571, 0.778258) -- (0.094082, 0.794973) -- (0.109592, 0.808486) -- (0.125102, 0.818576) -- (0.140612, 0.825077) -- (0.156122, 0.827883) -- (0.171633, 0.826946) -- (0.187143, 0.822284) -- (0.202653, 0.813971) -- (0.218163, 0.802145) -- (0.233673, 0.786999) -- (0.249184, 0.768783) -- (0.264694, 0.747796) -- (0.280204, 0.724382) -- (0.295714, 0.698925) -- (0.311224, 0.671845) -- (0.326735, 0.643584) -- (0.342245, 0.614608) -- (0.357755, 0.585392) -- (0.373265, 0.556416) -- (0.388776, 0.528155) -- (0.404286, 0.501075) -- (0.419796, 0.475618) -- (0.435306, 0.452204) -- (0.450816, 0.431217) -- (0.466327, 0.413001) -- (0.481837, 0.397855) -- (0.497347, 0.386029) -- (0.512857, 0.377716) -- (0.528367, 0.373054) -- (0.543878, 0.372117) -- (0.559388, 0.374923) -- (0.574898, 0.381424) -- (0.590408, 0.391514) -- (0.605918, 0.405027) -- (0.621429, 0.421742) -- (0.636939, 0.441384) -- (0.652449, 0.463631) -- (0.667959, 0.488116) -- (0.683469, 0.514439) -- (0.698980, 0.542167) -- (0.714490, 0.570844) -- (0.730000, 0.600000);
 

\draw[line width=0.046875cm, -latex] (1.250000, 3.680000) -- (1.250000, 4.680000);
 

\draw[line width=0.046875cm, -latex] (1.250000, 0.000000) -- (1.250000, 0.400000);
\draw[line width=0.046875cm, -latex] (1.250000, 0.800000) -- (1.250000, 2.130000);
 
\draw[line width=0.046875cm] (0.750000, 0.600000) -- (1.050000, 0.600000);
 
\draw[-latex, line width=0.046875cm, rounded corners=0.200000cm] (1.250000, 4.080000) -- (-0.750000, 4.080000) -- (-0.750000, 5.980000) -- (0.000000, 5.980000);
\draw[-latex, line width=0.046875cm, rounded corners=0.200000cm] (1.250000, 1.530000) -- (-0.750000, 1.530000) -- (-0.750000, 3.430000) -- (0.000000, 3.430000);
%\draw[-latex, line width=0.046875cm, rounded corners=0.200000cm] (5.250000, 1.530000) -- (7.250000, 1.530000) -- (7.250000, 3.830000) -- (6.500000, 3.830000); 

\draw[-latex, line width=0.046875cm, rounded corners=0.200000cm] (1.250000, 1.730000) -- (0.312500, 1.730000) -- (0.312500, 2.130000);
\draw[-latex, line width=0.046875cm, rounded corners=0.200000cm] (1.250000, 1.730000) -- (2.187500, 1.730000) -- (2.187500, 2.130000);

\draw[-latex, line width=0.046875cm, rounded corners=0.200000cm] (1.250000, 6.230000) -- (1.250000, 7.230000) -- (3.250000, 7.230000) -- (3.250000, 4.680000) -- (4.312500, 4.680000) -- (4.312500, 5.080000);
\draw[-latex, line width=0.046875cm, rounded corners=0.200000cm] (1.250000, 6.230000) -- (1.250000, 7.230000) -- (3.250000, 7.230000) -- (3.250000, 4.680000) -- (5.250000, 4.680000) -- (5.250000, 5.080000);

\draw[line width=0.046875cm, -latex] (1.250000, -1.500000) -- (1.250000, -0.900000);
 
\node[text width=2.500000cm, anchor=north, align=center] at (1.250000,-1.500000) {Inputs};

\node[text width=2.500000cm, anchor=south, align=center] at (1.250000,11.980000) {Output \vspace{-0.05cm} \linebreak Probabilities};
\node[anchor=east] at (-1.175000,3.880000) {$N\times$};

\node[text width=2.000000cm, anchor=east] at (0.250000,0.600000) {Positional \vspace{-0.05cm} \linebreak Encoding};

\end{tikzpicture}
